A Comprehensive Evaluation Framework for the Study of the Effects of Facial Filters on Face Recognition Accuracy

Facial filters are now commonplace for social media users around the world. Previous work has demonstrated that facial filters can negatively impact automated face recognition performance. However, these studies focus on small numbers of hand-picked filters in particular styles. In order to more effectively incorporate the wide ranges of filters present on various social media applications, we introduce a framework that allows for larger-scale study of the impact of facial filters on automated recognition. This framework includes a controlled dataset of face images, a principled filter selection process that selects a representative range of filters for experimentation, and a set of experiments to evaluate the filters' impact on recognition. We demonstrate our framework with a case study of filters from the American applications Instagram and Snapchat and the Chinese applications Meitu and Pitu to uncover cross-cultural differences. Finally, we show how the filtering effect in a face embedding space can easily be detected and restored to improve face recognition performance.

==> filter_selection_algorithm.tex <==
\begin{algorithm}
\caption{Filter Selection Process}\label{alg:framework}
\KwData{Base dataset $b$ of 1,000 subjects, 3 images per subject, filter application $a$, face recognition model $m$}
\KwResult{Filtered dataset $d$ with representative set of filters from $a$ applied}
$S \gets getFiltersSuperset()$\;
$P \gets selectRandomTenSubjectsPictures()$\;
\For{\texttt{s in S}}{
    \For{\texttt{p in P}}{
        \texttt{<apply each filter to every image, save output images in $L$>}}}


\For{$l$ in $L$}{
    $mean\_difference = l - original\_l$
    $binarized\_image = otsus(mean\_difference)$
    $manipulated\_pixels\_ratio = binarized\_image/image\_size$
    bin\_filter(manipulated\_pixels\_ratio)}

\SetKwProg{Fn}{Function}{}{}

\Fn{bin\_filter (manipulated\_pixels\_ratio)}{
 Group each filter into one of five bins by percentage of manipulated pixels: less than $20\%$, between $20\%$ and $40\%$, between $40\%$ and $60\%$, between $60\%$ and $80\%$ and greater than $80\%$
}

\For{$bin$ in $Bins$}{
    Select an equal number of filters per bin and apply these filters to all images in the dataset
}

\end{algorithm}

==> filtered_original_matching_algorithm.tex <==
\begin{algorithm}

\KwData{Facial embedding vectors of the unfiltered images (for original v. original) $O$ and of the images filtered with a filter $F$}
\KwResult{Genuine and Impostor Distributions}


\For{\texttt{o in O}}{
    \For{\texttt f in F}{
        \uIf{o and F are of the same subject}{
            \uIf{o and f' are not the same image}{
                Calculate cosine distance for genuine distribution
            }
        }
        \Else{
            Calculate cosine distance for impostor distribution
        }
    
    }
}
generateDistributionFromScores();
\vspace{5pt}
\caption{Algorithm for calculating genuine and impostor distributions from one-to-one matching for original image v. filtered image experiments}
\label{alg:filterd-experiment}
\end{algorithm}
%\vspace{-15pt}

==> original_matching_algorithm.tex <==
\begin{algorithm}

\KwData{Facial embedding vectors of either the unfiltered images (for original v. original) or set of images filtered with a single filter (filtered v. filtered), $F$}
\KwResult{Genuine and Impostor Distributions}


\For{\texttt{f in F}}{
    \For{\texttt f' in F}{
        \uIf{\texttt{f and f' have not been compared yet}} {
            \uIf{f and f' are of the same subject}{
                \uIf{f and f' are not the same image}{
                    Calculate cosine distance for genuine distribution
                }
            }
            \Else{
                Calculate cosine distance for impostor distribution
            }
    
        }
    }
}

generateDistributionFromScores();
\vspace{5pt}
\caption{Algorithm for calculating genuine and impostor distributions from one-to-one matching for baseline original image v. original image experiments and filtered image v. filtered image experiments for images with the same filter applied}\label{alg:orig-experiment}
\end{algorithm}


==> table_contributions_summary.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[]
\begin{center}
\begin{tabularx}{\textwidth}{|Y|Y|Y|Y|Y|Y|Y|Y|Y|Y|}
\hline
Authors & Controlled base image set & Standard biometrics methods & Filter types & Filter applications & Selects filters based on properties rather than popularity & Number of Filters\\
\hline
Botezatu \etal & Yes, FRGC (1441 subjects, 2882 images total) & Yes & Occlude & SweetFace Camera, B612, Snow, YouCam Fun, Bloom Camera & Yes & 10\\
\hline
Hedman \etal & No (4324 subjects) & Yes & Occlude and change color tones & Instagram & No & 8 \\
\hline
Mirabet-Herranz \etal & No (2026 base images) & Yes & Warp, change color tones & Instagram & No & 6\\
\hline
Riccio \etal & No (13000 and 108501 base images) & No & Warp, change color tones & Instagram & No & 8\\
\hline
Tiwari \etal & Yes, FRLL (102 subjects, 1020 images total) & No & All three & Snapchat, B612, FaceApp & Yes & 10\\
\hline
This Study & Yes, FRGC (1000 subjects, 3000 images total) & Yes & All three & Instagram, Snapchat, Meitu, Pitu & Yes & 125\\
\hline
\end{tabularx}
\end{center}
\caption{Summary of contributions of past work and our work. In addition to combining the best elements of prior work, our work additionally is the first of our knowledge to perform one-to-one and one-to-many experiments and consider the genuine/mated and impostor/nonmated distributions, the first of our knowledge to consider a large (at least 20 per platform, 125 across four platforms) number of filters, and the first to perform a cross-cultural comparision of American and Chinese filters. We also present a methodical filter selection method in this work.}
\label{tab:study_contributions}
\end{table}

==> table_dprime_flt_v_flt.tex <==
\begin{table}[h]
\centering
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\cline{3-6}
\multicolumn{2}{c|}{} & Bin 1. & Bin 2. & Bin 3. & Bin 4. \\
\cline{1-6}
\multirow{3}{*}{Instagram} & all & $8.47 \pm 2.24$
& $8.06 \pm 1.78$ & $9.32 \pm 1.5$ & $10.95 \pm 1.29$ \\
& female & $8.1 \pm 2.16$ & $7.7 \pm 1.74$ & $8.96 \pm 1.52$ & $10.59 \pm 1.26$ \\
& male & $8.18 \pm 2.34$ & $7.81 \pm 1.85$ & $9.12 \pm 1.49$ & $10.75 \pm 1.23$ \\
\cline{1-6}
\multirow{3}{*}{Snapchat} & all & $8.43 \pm 2.06$
& $5.97 \pm 2.78$ & $-$ & $-$ \\
& female & $8.12 \pm 2.05$ & $5.67 \pm 2.7$ & $-$ & $-$ \\
& male & $8.13 \pm 2.04$ & $5.69 \pm 2.72$ & $-$ & $-$ \\
\cline{1-6}
\multirow{3}{*}{Meitu} & all & $9.31 \pm 0.66$
& $9.5 \pm 0.56$ & $9.39 \pm 0.69$ & $9.4 \pm 0.56$ \\
& female & $8.82 \pm 0.7$ & $9.12 \pm 0.59$ & $8.88 \pm 0.73$ & $9.09 \pm 0.73$ \\
& male & $9.27 \pm 0.77$ & $9.33 \pm 0.56$ & $9.38 \pm 0.69$ & $9.2 \pm 0.58$ \\
\cline{1-6}
\multirow{3}{*}{Pitu} & all & $9.81 \pm 0.33$
& $-$ & $9.59 \pm 0.38$ & $9.79 \pm 0.59$ \\
& female & $9.47 \pm 0.53$ & $-$ & $9.58 \pm 0.64$ & $9.58 \pm 0.71$ \\
& male & $9.69 \pm 0.39$ & $-$ & $9.17 \pm 0.52$ & $9.53 \pm 0.47$ \\
\cline{1-6}
\end{tabular}
\end{center}
\caption{D-prime values between genuine and impostor distributions for filtered v. filtered images.}
\label{tab:dprime_flt_v_flt_sup}
\end{table}
